EASYFLOW: Keep Ethereum Away From Overflow

While Ethereum smart contracts enabled a wide range of blockchain applications, they are extremely vulnerable to different forms of security attacks. Due to the fact that transactions to smart contracts commonly involve cryptocurrency transfer, any successful attacks can lead to money loss or even financial disorder. In this paper, we focus on the overflow attacks in Ethereum , mainly because they widely rooted in many smart contracts and comparatively easy to exploit. We have developed EASYFLOW , an overflow detector at Ethereum Virtual Machine level. The key insight behind EASYFLOW is a taint analysis based tracking technique to analyze the propagation of involved taints. Specifically, EASYFLOW can not only divide smart contracts into safe contracts, manifested overflows, well-protected overflows and potential overflows, but also automatically generate transactions to trigger potential overflows. In our preliminary evaluation, EASYFLOW managed to find potentially vulnerable Ethereum contracts with little runtime overhead.

==> data/figure_safeadd.tex <==
\begin{figure}[h]
\begin{lstlisting}[frame=none, numbers=left, language=Java, showstringspaces=false, morekeywords={function,contract,uint,mapping,address,event,bytes,uint256}]
function add(uint256 a, uint256 b) internal pure 
                           returns (uint256) {
  uint256 c = a + b;
  require(c >= a);
  return c;
}
\end{lstlisting}
\caption{A function of SafeMath Library}
\label{figure:safeadd}
\end{figure}

==> data/overview.tex <==
%To begin with, we introduce the general framework of \tool. 
%We mainly explain the key modules and their interactions. The framework is shown 
%in Figure~\ref{fig:framework}.



Generally, \tool takes as input the software under test (SUT), 
including class files, jar and war packages. 
In terms of output, \tool 
generates a bug report including specific types of bugs found 
in the analysis and runtime coverage information which helps users 
better understand the results and tune the analysis. Currently, \tool 
is able to detect four common types of concurrency bugs, \ie, 
assertion failures, data races, 
deadlocks and null pointer dereferences. 
Since the main strength of \tool is to efficiently cover both 
thread interleaving and program paths rather than the detection itself, 
we implement well-designed detection algorithms in \tool. 
Specifically, we check assert exceptions to capture assertion failures. 
Data races and deadlocks are detected using the FastTrack~\cite{Flanagan:2009:pldi} 
and GoodLock~\cite{havelund2000using} algorithms, respectively. In terms of null pointer 
dereferences, we extend FastTrack by dumping heap memory involved in a data race 
and flag a bug if the race incurs a read operation and the memory value is \texttt{null}.

%Furthermore, 
%\tool allows developers to make extensions by designing new analysis 
%for specific use cases.
%
%
%For classes compiled 
%with the debugging option opened, \tool can give 
%files and reports concurrency 
%bugs found during the dynamic analysis process. 
%
%\myparagraph{Input}
%Specifically, allowed types of input are listed below. 
%Both types need at least a \texttt{main()} entry.
% 
%\begin{itemize}[leftmargin=*]
%	\item multithreaded \texttt{.class} files
%	\item multithreaded \texttt{jar} file
%\end{itemize}

%
%\myparagraph{Output} 
%The \tool detects the following types of bugs, each of which 
%is labeled by a CWE ID. 
%
%\begin{itemize}[leftmargin=*]
%\item CWE 362-367: race conditions
%\item CWE 662, 667: Atomicity violations
%\item CWE 833: Deadlock
%\item CWE 617: Fatal assertions
%\item CWE 476: Null pointer deferences
%\item CWE 248: Uncaught exceptions
%\end{itemize}



The architecture of \tool is shown in Figure~\ref{fig:framework}. 
Specifically, \tool works in three modes, \ie, schedule fuzzing mode, symbolic 
trace analysis mode and bug detection mode. Generally, the schedule fuzzing mode aims at 
efficiently exploring the state space based on observed traces. Differently, 
the symbolic trace analysis mode tries to infer the existence of possible unobserved paths 
and drive the execution to cover them. Lastly, the bug detection mode targets at 
capturing various types of concurrency bugs. Specifically, \tool consists of 
six modules, \ie, \emph{Schedule fuzzer}, \emph{Scheduler}, 
\emph{Profiler}, \emph{Branch finder}, \emph{SMT solver} and 
\emph{Bug detector}. Next, we describe the general workflow of \tool and 
interaction among modules.


First, the \emph{Schedule fuzzer} aims at fuzzing 
thread schedules. To this end, it runs the program and randomly generates a set of 
priority change (PC) points in the program. At PC points, context 
switches are enforced. At non-PC points, the thread which 
owns the CPU will proceed. Then, \emph{Scheduler} leverages the computed schedule to 
execute threads and produce runtime traces. Based on a trace, 
a \emph{Bug detector} checks whether specific types of bugs occur or not. 
At the same time, \emph{Profiler} computes the coverage information as a feedback 
to the \emph{Schedule fuzzer}. In our setting, we mainly consider the 
define-use coverage metric~\cite{lu2007study}. This metric is suitable for detecting 
memory access related bugs, which is a majority in real-world applications. The 
coverage information serves as a guidance to help the \emph{Schedule fuzzer} 
better generate new schedules in iterative runs. 
%Moreover, \tool keeps monitoring the change of runtime coverage, 
%and identifies the saturation of the fuzzing process. 
%%When the seen change is less than a threshold for a specified number of iterations, 
%%\tool considers the fuzzing has come to a saturation. 
%In that case, \tool 
Moreover, \tool 
switches to the symbolic trace analysis mode when fuzzing saturates. 
A \emph{Branch finder} is notified to find schedule sensitive branches~\cite{huang2015finding} 
based on previously collected traces. 
To do that, it builds a set of constraints of event ordering and memory dependency. 
The constraints are passed to a \emph{SMT solver} to check satisfiability. 
For unsatisfiable results, we ignore the trace. In terms of satisfiable ones, 
which indicate that specific event ordering can pick an unexplored path of the branch, 
we generate a solution to the constraints and leverage the \emph{Schedule fuzzer} 
to enforce the computed schedule of the solution. 


\subsection{Key Insight}
%\myparagraph{Key Insight}
To hunt deep concurrency bugs and make \tool practically useful, 
%To improve the efficiency and scalability of \tool in finding concurrency 
%bugs, 
our design adopts the following key optimizations and insights.

\myparagraph{Combined Analysis Engine}
\tool employ a dynamic transition between schedule fuzzing and symbolic trace analysis 
modes, which enables bug detection in a relatively lightweight manner (schedule fuzzing) 
and at the same time stays sensitive to control flow structure as much as possible (symbolic trace 
analysis).

\myparagraph{Stochastic Schedule Fuzzing}
In the schedule fuzzing mode, \tool enables stochastic optimizations on schedule fuzzing. 
Memory accesses from a thread are put into groups such that the number of scheduling 
points get reduced. A memory access group does not allow write-read or write-write 
to the same memory location. To schedule the program at a group granularity, 
\tool uses a bool vector $\mathcal{X} = \langle x_1, x_2, \cdots, x_k\rangle$ to specify 
whether group $i$ generates a context switch. At each iteration, \tool 
leverages Markov Chain Monte Carlo (MCMC) to propose and accept a new vector 
based on the current $\mathcal{X}$. The proposal randomly flips a small number of 
values in $\mathcal{X}$. Using the coverage to encode the objective function, 
\tool accepts the proposal with a specific probability.

\myparagraph{Symbolic Trace Analysis}
In the symbolic trace analysis mode, the goal of \tool is to identify schedule sensitive 
branches~\cite{huang2015finding} and steer the execution to find 
unexplored paths. To this end, \tool constructs a set of constraints 
based on runtime traces, \ie, program order (PO), synchronization order (SO), 
memory dependency (MD) and branch condition (BC). Specifically, PO 
requires operations from the same thread are ordered as in traces. SO 
defines partial orders on synchronizations, \eg, \texttt{fork}, 
\texttt{lock}, \texttt{unlock}, \texttt{wait}, \texttt{notify} \etc. 
MD says that a read memory access gets the value from the most recent write. 
BC is the set of predicates of branches. For explicit branches as \texttt{if-else}, 
\tool uses the branch condition as BC. For implicit branches as exception handling, 
\tool predefined patterns to indicate the condition of exception, \eg, divide by zero, 
out-of-bound access \etc. Based on the collected constraints, \tool leverages an 
SMT solver to check whether they are satisfiable. If so, \tool generates a feasible 
solution as the new schedule.

%\begin{itemize}[leftmargin=*]
%\item We employ a dynamic transition between fuzzing and symbolic trace analysis 
%techniques, which can detect bugs in a relatively lightweight manner (fuzzing) 
%and stay sensitive to control flow structure as much as possible (symbolic trace 
%analysis).
%
%\item We perform two-fold optimizations on schedule fuzzing. First, we reduce 
%the number of random context switches at operations less likely to trigger 
%concurrency bugs. Second, we leverage coverage as feedback to search for 
%better schedules iteratively. 
%
%\item We identify both explicit (\texttt{if-else} like branches) and 
%implicit (exception handling routines) schedule sensitive 
%branches by extracting and solving different types of constraints via the 
%symbolic trace analysis.  
%\end{itemize}
%
%Based on the general workflow, we next introduce the key insight of \tool, 
%\ie, dividing programs into \emph{rooms} and \emph{doors}. Conceptually, 
%we regard SSBs as \emph{doors} which determine the executed path based on 
%a specific schedule. \emph{Rooms} are code blocks between two consecutive 
%\emph{doors}. We use the example in Figure~\ref{fig:framework} to explain the 
%concepts. Specifically, there are two \emph{doors} in the given example marked as 
%$D_1$ (line 9) and $D_2$ (line 14). $D_1$ is an implicit SSB since it is not within 
%an \texttt{if-else} branch. It operates a division where a divide-by-zero 
%exception may be thrown due to some buggy schedule. In this case, if line 17 
%executed before line 9 and after line 3. The variable \texttt{y} will be set to 
%0 and triggers the exception. Consequently, the \texttt{catch} path will be 
%picked. Another \emph{door} $D_2$ is an explicit SSB where the condition 
%\texttt{x == 0} is dependent on schedules. For example, if line 18 executes 
%before line 14 and after line 8 (\texttt{catch} is not run), $D_2$ will 
%take the path at line 15 and thus trigger an assertion failure bug. Using 
%$D_1$ and $D_2$ as two split lines, the program is then divided into five 
%\emph{rooms}, \ie, $R_i, i=1\cdots5$. Inside a \emph{room}, there is no 
%\emph{doors}. Some \emph{rooms} are usually invisible at the very beginning 
%if the guarding \emph{door} is not opened. In this case, only $R_1$ and 
%$R_5$ can be easily visited. The execution of $R_2$ and $R_3$ is dependent on 
%$D_1$. Similarly, $R_4$ can only be explored if the \texttt{true} path of $D_2$ 
%is picked. Commonly, the number of interleaving of inner-room events are 
%quite large in practice. \tool aims at efficiently fuzzing each \emph{room} to 
%find bug-triggering schedules and further search for more \emph{rooms} 
%through analyzing \emph{doors}. In the following sections, we first illustrate 
%how to better fuzz \emph{rooms} (\S\ref{subsec:mag}). Then, we discuss on 
%symbolic analysis based technique to find and open \emph{doors} (\S\ref{subsec:sta}). 
%Finally, we explain the transition between fuzzing and symbolic analysis 
%process (\S\ref{subsec:switch}).

%\begin{figure}
%\begin{lstlisting}[frame=none, numbers=left, language=Java, showstringspaces=false]
%x = 0; y = 0;
%Thread t1:
%  y = 2;
%  try {
%    fork t2;
%    lock m;
%    z = x + y;
%    x++;
%    z = z / y;
%    unlock m;
%  } catch {
%    x = 1;
%  }
%  if(x == 0) 
%    assert(false);
%Thread t2:
%  y = 0;
%  x = 0;
%\end{lstlisting}
%\caption{Two different types of SSB.}
%\label{fig:overview:example}
%\end{figure}

==> data/preamble.tex <==
\usepackage{booktabs} % For formal tables

\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{balance} 
\usepackage{amssymb}
\usepackage{xspace}
\usepackage[T1]{fontenc}
\usepackage[scaled=0.81]{beramono}
\usepackage{balance}
\let\labelindent\relax
\usepackage{enumitem}  
\usepackage{listings}
\usepackage{url}
\usepackage[ruled,lined,linesnumbered,vlined]{algorithm2e}
\usepackage{multirow}
\usepackage{array}

\usepackage{url}
\def\UrlBreaks{\do\0\do\1\do\2\do\3\do\4\do\5\do\6\do\7\do\8\do\9\do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X\do\Y\do\Z\do\/\do\.\do\-\do\:}

\usepackage{color}
\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.13}

\lstset{
	basicstyle=\ttfamily\small,
	%	numbers=left,
	xleftmargin=2em,
	%	numbersep=0.1pt,
	keywordstyle=\color{blue},
	commentstyle=\color{darkgreen},
}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Macros																{{{1
% Terminology
\newcommand{\tool}{\hbox{\textsc{EasyFlow}}\xspace}
\newcommand{\ethereum}{\hbox{Ethereum}\xspace}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}

% Command
\newcommand{\myparagraph}[1]{\vspace*{0.14cm}\noindent\textbf{#1.}\quad}
\newtheorem{thm}{Theorem}
\newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

% English
\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\scil}{\hbox{\emph{sc.}}\xspace} %scilicet: it is 
%permitted to know
%\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace} %videlicet: it is 
%permitted to see

\newcommand{\toolUrl}{\texttt{\url{XXX}}} 
\newcommand{\videoUrl}{\texttt{\url{XXX}}}



